Multiple Source Replacement Path Problem

One of the classical line of work in graph algorithms has been the Replacement Path Problem: given a graph $G$, $s$ and $t$, find shortest paths from $s$ to $t$ avoiding each edge $e$ on the shortest path from $s$ to $t$. These paths are called replacement paths in literature. For an undirected and unweighted graph, (Malik, Mittal, and Gupta, Operation Research Letters, 1989) and (Hershberger and Suri, FOCS 2001) designed an algorithm that solves the replacement path problem in $\tilde O(m+n)$ time. It is natural to ask whether we can generalize the replacement path problem: {\em can we find all replacement paths from a source $s$ to all vertices in $G$?} This problem is called the Single Source Replacement Path Problem. Recently (Chechik and Cohen, SODA 2019) designed a randomized combinatorial algorithm that solves the Single Source Replacement Path Problem in $\tilde O(m\sqrt n\ + n^2)$ time. One of the questions left unanswered by their work is the case when there are many sources, not one. When there are $n$ sources, the combinatorial algorithm of (Bernstein and Karger, STOC 2009) can be used to find all pair replacement path in $\tilde O(mn + n^3)$ time. However, there is no result known for any general $\sigma$. Thus, the problem we study is defined as follows: given a set of $\sigma$ sources, we want to find the replacement path from these sources to all vertices in $G$. We give a randomized combinatorial algorithm for this problem that takes $\tilde O(m\sqrt{n \sigma} +\ \sigma n^2)$ time. This result generalizes both results known for this problem. Our algorithm is much different and arguably simpler than (Chechik and Cohen, SODA 2019). Like them, we show a matching conditional lower bound using the Boolean Matrix Multiplication conjecture.

==> application.tex <==

\section{Application of Our Result: Fault Tolerant Exact Distance Oracle}
\begin{comment}
Our result has many application in related problem. We note few of them in this section.

\begin{enumerate}
\item {\bf Single Edge Fault Tolerant Subgraph Problem}: In this problem, we need to
find a subgraph $H$ of $G$ such that all the replacement
paths from $s \in \SSS$ to $t \in V$ are preserved in $H$. Formally, if
$P(s,e,t)$ is the shortest path from a source $s$ to a destination $t$ avoiding
$e$, then $P(s,e,t)$ lies in $H$. Thus, $H = \cup_{s \in \SSS,t\in
V,e \in E} P(s,e,t)$. Parter and Peleg \cite{Parter2013} showed that there always exists a subgraph $H$ os size $O(\sigma^{1/2}n^{3/2})$. Moreover, they give an unspecified polynomial time algorithm for this problem. We apply our techniques to show the following:

\begin{lemma}
There exists a randomized  algorithm that can find a single fault tolerant subgraph $H$ of  $G$ in $\tilde O(m \sqrt n+n^{2})$ time.
\end{lemma} 
\end{comment}
  Consider the following problem in which we need to
build a data-structure that will answer the following query:
\textsc{Query}($s,t,e$): Find the shortest path from $s$
to $t$ avoiding $e$, where $s \in \SSS$, $t \in V$ and $e \in E$. Gupta and Singh\cite{GuptaS18} showed that there exists a data-structure of size $\tilde O(\sigma^{1/2}n^{3/2})$ that can answer queries in $\tilde  O(1)$ time. In their paper, this data-structure can be constructed in (unspecified) polynomial time. We use our techniques to show that following:

\begin{lemma}
There exists a randomized algorithm that construct a exact single fault tolerant distance oracle in $\tilde O(m\sqrt{ n\sigma}+\sigma n^{2})$ time such that after construction each query can be answer in $\tilde O(1)$ time.
\end{lemma}






\begin{comment}
All the above problems have been studies before when there
is a single fault. However, none of the previous work discuss
about efficient algorithm to  solve the problem. For example,
in the subgraph problem, even though we know that  a subgraph
$H$ of size $O(n^{3/2})$ exists, we don't know how to find
that subgraph efficiently. For the distance oracle, we know
that a distance oracle of size $\tilde O(n^{3/2})$ exists
that can answer queries in $\tilde O(1)$ time. But we don't
know how to find that oracle efficiently.

Our work fills this void. We show that all the above problem
can be solve in $\tilde O(mn)$ time.


\subsection{Single Edge Fault Tolerant Subgraph}
Given a graph $G$, we want to find a subgraph $H$ of $G$ such that all the replacement path from $s$ to $t \in V$ are preserved in $G$. Parter and Peleg \cite{Parter2013} showed that there always exists a subgraph $H$ with size $O(n^{3/2})$. We now describe their algorithm. 

\begin{algorithm}[H]



\ForEach{$s \in \SSS}
{
\ForEach{$t \in V$}
{
   
   \ForEach{ $e \in st$ path}
   {
       $P_e \leftarrow$ the replacement path from $s$ to $t$ avoiding $e$\;
       Add the last edge of $P_e$ to $H$.
   }
}
}
\end{algorithm}

The above algorithm adds the last edge of all replacement paths to the subgraph $H$.
We assume that all the replacement path are unique. This can be done by perturbing edge weights (as we had done in Section \ref{}). Fix a $t \in V$. We want to find the number of distinct edges added by the above algorithm to $t$. To formalize this, let us define the notion of contributing edges.

\begin{definition}
A replacement path $P$ is said to be contributing if it adds a new edge to $t$ in $H$.
\end{definition}

In \cite{Parter2013}, the authors then show the following 

\begin{lemma}
The number of contributing edges to from a source $s$ $t$ is $O(\sigma\sqrt n)$.
\end{lemma}
The proof of this lemma hinges on the fact that for all such replacement path, their $\SUF(\cdot)$ is disjoint. Also, the length of $\SUF(\cdot)$ is distinct for distinct replacement paths. One can see that by counting argument there can be atmost $O(\sqrt n)$ many replacement paths.

Even though the above algorithm and the analysis is elegant, the algorithm --- as it is right now --- takes polynomial time. The main bottle neck for this algorithm is finding the replacement path for each edge $e \in st$. We now use our techniques to fill this gap.  

Let us first look at the case of near edges. Using Lemma \ref{lem:gs18}(3), we know that there are $\sqrt n$ contiguous
blocks of edges in $st_s$ path such that the length of a
replacement path for all the edges in a block is same. In Section \ref{sec:near}, we saw that for each $e \in st_s$ , we can find the shortest path from edges in each block in $O(m \sqrt n + n^2)$ time. Note that even though we are finding the length of the replacement path in our algorithm, the suffix of this replacement path is a shortest path from a vertex in $\RR$ to $t$. Thus, whenever we find the shortest path for a block of vertices, we add the corresponding last edge from a vertex from $\RR$ to $t$ in $H$. Since
there are at most $\sqrt  n$ such blocks, the total number of vertices added by our algorithm is $O(\sqrt n)$.

Now, consider the case when we are processing a near edge $e$. If $|st \diamond e| \le |st| +c \sqrt n \log n$, then look  at place in Algorithm \ref{alg:main} when we set $d(s,t,e)$. There must be a vertex $v$ such that extending the path $sv \diamond e'$ gives us $st \diamond e$. Note that here $e'= \emptyset$ or $e' = e$. Thus, whenever we set the distance $d(s,t,e)$, we add the corresponding edge $(v,t)$ in the subgraph $H$. Since, we have already established that the number of contributing edges are at most $O(\sqrt n)$, the total number of edges added in this case is also $O(\sqrt n)$. 

If $d(s,t,e) \ge |st| + c\sqrt n \log n$, then again there exists a vertex $r \in \RR$ such that the suffix of the replacement path is the shortest path from $r$ to $t$. Thus, for each such $e \in t_st$ path, we find the corresponding $r$ and add the last edge on this path to $H$. Again the total number of edges added in this case is $O(\sqrt n)$. 

Since, the total time taken to find all the paths is $\tilde O(m \sqrt n + n^2)$, the total running time of our algorithm to find the subgraph $H$ is $\tilde O(m\sqrt n + n^2)$.
\end{comment}

\subsection{Single Source Case: when $\sigma=1$}

In \cite{GuptaS18}, the authors showed that there exists a single fault tolerant distance oracle of size $\tilde O(n^{3/2})$ such that queries can be answered in $\tilde O(1)$ time. We first give an overview of the data-structure used in \cite{GuptaS18}.

Fix a vertex $t$. We first find the corresponding $t_s$. For each edge $e \in st$, the replacement path may pass through $t_s$. In such a case, we have already calculated $d(s.t_s,t)$ and $d(t_s,t)$. Thus, we have two data-structure: 1) A hash-table which stores all the replacement paths from $s$ to $r \in \RR$ avoiding all edges in $sr$ path  and 2) A hash-table which stores the shortest path from $r \in \RR$ and $t \in V$. The first data-structure takes $\tilde O(n^{3/2})$ space as $|\RR| = O(n^{3/2})$.  The second dictionary also takes $O(n^{3/2})$  space. Thus, if the replacement path passes through $t_s$, we can find it in $O(1)$ time. 

Let us now look at the case when $e \in st_s$ and the replacement
path avoids $t_s$. For this case, we use the Lemma \ref{lem:gs18},
which says that there are at most $\sqrt n$ such replacement
paths from $s$ to $t$ that avoid $t_s$ too and these replacement paths avoid a contagious sequence
of edges in $st_s$ path.
In fact our modified algorithm in Section \ref{sec:modified} finds all the replacement path that avoid $t_s$ too. 

Let the replacement path $P$ avoids the some contiguuous subpath in $st_s$. 
Let $f(P)$ and $\l(P)$ denote the first and the last
vertex of the contiguous path that $P$ avoids. Given a vertex
$v$, let $v.depth$ denote the depth of $v$ in the BFS tree
of $s$.  We can store the depth of all the vertices in an
array (takes $O(n)$ space).



We build a balanced
binary search tree\ BST($t$) in which each node represents
a path $P$. The key used to search the node is the range:
$[ f(P).depth,  l(P).depth]$. By Lemma \ref{lem:gs:18}(3),
all the replacement paths avoid  contiguous subpaths of
$st_s$.  These contiguous subpaths are also disjoint as there
is only one replacement path avoiding an edge. Thus, the key
we have chosen form a total ordered set with respect to
the relation $\{ <,>\}$.  The size of BST($t$) is $O(\sqrt
n)$ as the size of $\RR$ is $O(\sqrt n)$. Thus, the total space taken by the data-structure is $\tilde O(n^{3/2})$. If the replacement path from $s$ to $t$ avoiding $e \in st_s$ avoids $t_s$ too, then we can find by searching the range in with $e$ lies in $\BST(t)$. Thus, the time to find the replacement path is $\tilde O(1)$ (for this case also).

For a fixed $t$, the extra work of building the $\BST(t)$ is $\tilde O(\sqrt n)$, totalling to $\tilde O(n\sqrt n)$ overall. We disregard this term as it is asymptotically smaller than our overall running time.


Let us now look at the case when $e \in t_st$ (that is far edges). For all the $\tilde O(\sqrt n)$ edges in $t_st$, out algorithm finds the length of their replacement paths in $\tilde O(m\sqrt n+n^2)$ time. For each $e \in t_st$, we keep it corresponding replacement path in a hash-table. For a fixed $t$, the size of our data-strcuture is $\tilde O(\sqrt n)$ as $|t_st| = \tilde O(\sqrt n)$. Thus, the total size of our data-structure is $\tilde O(n^{3/2})$. As far as query is concerned, it takes $O(1)$ time to find if $e \in t_st$. Then we can use our hash-table to find the replacement path avoiding $e$. Thus, the time taken to find the replacement path in this case is $O(1)$. 

The reader can check that all of our data-structure is of size $\tilde O(n^{3/2})$. Moreover, the tie taken to build the data-structure is $\tilde O(m\sqrt n + n^2)$ and the query time is $\tilde O(1)$.
\
 





==> conclusion.tex <==
\section{Conclusion and Further Work}
In this paper, we designed a simple algorithm that solves the $\SSR$ problem in $\TL(m\sqrt n +  n^2)$.
time. This algorithm can also be
extended to solve $\MSR$ problem with a running time of $\TL(m\NS + \SI n^2)$. Further, we showed a conditional lower bound of $\Omega(m\NS)$ for the $\MSR$ problem.

%One of the main open questions is that: {\em is the last term in the running time of $\MSR$ necessary}.
%Our conditional lower bound result does not rule out this possibility. Bridging this gap would be a challenging problem.
